3D Point Cloud Network Pruning: When Some Weights Do not Matter

A point cloud is a crucial geometric data structure utilized in numerous applications. The adoption of deep neural networks referred to as Point Cloud Neural Networks (PC- NNs), for processing 3D point clouds, has significantly advanced fields that rely on 3D geometric data to enhance the efficiency of tasks. Expanding the size of both neural network models and 3D point clouds introduces significant challenges in minimizing computational and memory requirements. This is essential for meeting the demanding requirements of real-world applications, which prioritize minimal energy consumption and low latency. Therefore, investigating redundancy in PCNNs is crucial yet challenging due to their sensitivity to parameters. Additionally, traditional pruning methods face difficulties as these networks rely heavily on weights and points. Nonetheless, our research reveals a promising phenomenon that could refine standard PCNN pruning techniques. Our findings suggest that preserving only the top p% of the highest magnitude weights is crucial for accuracy preservation. For example, pruning 99% of the weights from the PointNet model still results in accuracy close to the base level. Specifically, in the ModelNet40 dataset, where the base accuracy with the PointNet model was 87. 5%, preserving only 1% of the weights still achieves an accuracy of 86.8%. Codes are available in: https://github.com/apurba-nsu-rnd-lab/PCNN_Pruning

==> figs/un.tex <==

\begin{table}[!t]
    \captionsetup{skip=5pt} % Adjust the vertical spacing between caption and table
    \centering
    \scalebox{.67}{
        \begin{tabular}{l c c *{4}{c} *{4}{c} *{4}{c}} 
            \toprule
            \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{PR}} & \multirow{2}{*}{\textbf{Params(M)}} & \multicolumn{4}{c}{\textbf{ModelNet40}} & \multicolumn{4}{c}{\textbf{ScanObjectNN}} & \multicolumn{4}{c}{\textbf{ShapeNetCore}} \\ % Removed a column for parameters
            \cmidrule{4-7} \cmidrule{8-11} \cmidrule{12-15}
            & & & \textbf{IMP} & \textbf{IMP\_L} & \textbf{OneShot} & & \textbf{IMP} & \textbf{IMP\_L} & \textbf{OneShot} & & \textbf{IMP} & \textbf{IMP\_L} & \textbf{OneShot} & \\
            \midrule
            PointNet & 0 & 3.4 & 87.5 & 87.5 & 87.5 & & 65.0 & 65.0 & 65.0 & & 83.1 & 83.1 & 83.1 \\ % No bold formatting for numeric values
            & 60 & 1.36 & \textbf{88.7} & 88.4 & 88.0 & & 63.5 & 62.8 & \textbf{65.4} & & \textbf{84.9} & 84.5 & 84.3 \\ % No bold formatting for numeric values
            & 99 & 0.034 & 87.1 & 8.7 & 86.8 & & 64.7 & 32.1 & 62.7 & & 84.5 & 25.3 & 83.1 \\ % No bold formatting for numeric values
            \midrule
            DGCNN    & 0 & 1.7 & 89.2 & 89.2 & 89.2 & & 71.4 & 71.4 & 71.4 & & 82.1 & 82.1 & 82.1 \\ % No bold formatting for numeric values
            & 60 & 0.68 & \textbf{89.7} & 89.3 & 89.5 & & \textbf{75.7} & 73.6 & 75.5 & & \textbf{83.2} & 82.2 & 82.5 \\ % No bold formatting for numeric values
            & 99 & 0.017 & 86.3 & 65.2 & 86.2 & & 72.5 & 52.6 & 60.5 & & 80.5 & 72.5 & 79.8 \\ % No bold formatting for numeric values
            \midrule
            PointCNN & 0 & 0.32 & - & - & - & & - & - & - & & - & - & - \\
            & 60 & 0.128 & - & - & - & & - & - & - & & - & - & - \\
            & 90 & 0.032 & - & - & - & & - & - & - & & - & - & - \\
            \bottomrule
        \end{tabular}
    }
    \caption{\small Example}
    \label{tab:result}
\end{table}


\begin{figure}[!t]
    \centering
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/plot.pdf}
        %\caption{}
        %\label{fig:pointnet_dgcnn_prune}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/plot_weight1.pdf}
        %\caption{}
        %\label{fig:weight_dgcnn_pointnet}
    \end{minipage}
    \caption{\small \SR{to increase font size a bit, add the tnse and then a table as we discussed. Do it quickly. I have a meeting with Ali
    }}
    \label{fig:ablation}
\end{figure}

